Imaginary-time Mpemba effect in quantum many-body systems

Various exotic phenomena emerge in non-equilibrium quantum many-body systems. The Mpemba effect, denoting the situation where a hot system freezes faster than the colder one, is a counterintuitive non-equilibrium phenomenon that has attracted enduring interest for more than half a century. In this Letter, we report a novel phenomenon of the Mpemba effect in the imaginary-time relaxation dynamics in quantum many-body systems, dubbed as imaginary-time Mpemba effect (ITME). Through numerically exact quantum Monte-Carlo (QMC) simulation, we unambiguously demonstrate that in different classes of interacting quantum models, the initial states with higher energy are relaxed faster than lower-energy initial states in the process of imaginary-time relaxation. The emergence of ITME is intimately associated with the low-energy excitations in quantum many-body systems. More crucially, since imaginary-time dynamics is broadly applied in numerical simulation on the quantum many-body ground states, the discovery of ITME potentially provides a new pathway to expedite the quantum many-body computation, particularly for QMC involving the sign problem.

==> name.tex <==
To better understand the absence of ITME, we perform analytical analysis for the initial states with varying amplitudes of MF ordering field in the non-interacting Dirac-fermion systems. We consider a lattice model featuring Dirac fermions with periodic boundary conditions. Owing to the lattice translational symmetry, we can diagonalize the Hamiltonian in the space of lattice momentum. For example, for the tight-binding model involving NN hopping on the honeycomb lattice, the Hamiltonian reads: 
\bea
H_0 = -t \sum_{\avg{ij}} c^\dagger_{i,A} c_{j,B} + h.c.,
\label{NIHam1}
\eea
where $c^\dagger_{i,A(B)}$ denotes the creation operator of an electron on the site $i$ of the $A(B)$ sub-lattice, and $t$ is the amplitude of the NN hopping. After Fourier transform of the fermion operator by $c^\dagger_{i,A(B)} = \frac{1}{N} \sum_{\vec{k}} e^{i\vec{k}\cdot \vec{r}_i}c_{\vec{k},A(B)}$ where $N$ is the total number of unit cell and $\vec{k}$ is the lattice momentum belonging to the first Brillouin zone,  the Hamiltonian in the lattice-momentum space is $H_0 = \sum_{\vec{k}} H_0(\vec{k}) = \sum_{\vec{k}} \psi^\dagger_{\vec{k}} h_0(\vec{k}) \psi_{\vec{k}}$, where we introduce the two-component vector $\psi_{\vec{k}} = (c_{\vec{k},A},c_{\vec{k},B})$. The kernel matrix $h_0(\vec{k})$ is expressed as:
\begin{equation}
\label{S7}
h_0(\vec{k})=
\begin{pmatrix}
0 & -t(e^{i\vec{\delta}_1\cdot\vec{k}}+e^{i\vec{\delta}_2\cdot\vec{k}}+e^{i\vec{\delta}_3\cdot\vec{k}}) \\
-t(e^{-i\vec{\delta}_1\cdot\vec{k}}+e^{-i\vec{\delta}_2\cdot\vec{k}}+e^{-i\vec{\delta}_3\cdot\vec{k}}) & 0
\end{pmatrix}
\end{equation}
where $\vec{\delta}_1 = (0,1)$, $\vec{\delta}_2 = (\frac{\sqrt{3}}{2},-\frac{1}{2})$ and $\vec{\delta}_3 = (-\frac{\sqrt{3}}{2},-\frac{1}{2})$ represents the three vectors of NN bond on the honeycomb lattice. The eigenvalues of $H_0(\vec{k})$ is $\epsilon_{\pm}(\vec{k}) = \pm 2t\sqrt{3+(\cos[(\vec{\delta}_1-\vec{\delta}_2)\cdot \vec{k}]+\cos[(\vec{\delta}_1-\vec{\delta}_3)\cdot \vec{k}]+\cos[(\vec{\delta}_2-\vec{\delta}_3)\cdot \vec{k}])}$, and the associated single-particle eigenstate is denoted as $\alpha^\dagger_{\pm}(\vec{k})\ket{0}$.  

In the main text, we consider the initial states of MF ordering wave function, which is generated as the ground state of the non-interacting Hamiltonian involving MF ordering field. Without the loss of generalization, we consider the CDW MF ordering in the non-interacting Hamiltonian of \Eq{NIHam1}:
\bea
H_{MF} = H_0 + \sum_i \delta_i M_c, 
\label{MFHam1}
\eea
where $M_c$ is the amplitude of the CDW ordering field and $\delta_i = 1(-1)$ if site $i$ belongs to the A(B) sub-lattice. In the momentum space, the Hamiltonian $H_{MF} = \sum_{\vec{k}} H_{MF}(\vec{k}) = \sum_{\vec{k}}  \psi^\dagger_{\vec{k}} h_{MF}(\vec{k}) \psi_{\vec{k}} $, with the associated kernel matrix $h_{MF}(\vec{k})$ expressed as:
\begin{equation}
\label{S7}
h_{MF}(\vec{k})=
\begin{pmatrix}
M_c & -t(e^{i\vec{\delta}_1\cdot\vec{k}}+e^{i\vec{\delta}_2\cdot\vec{k}}+e^{i\vec{\delta}_3\cdot\vec{k}}) \\
-t(e^{-i\vec{\delta}_1\cdot\vec{k}}+e^{-i\vec{\delta}_2\cdot\vec{k}}+e^{-i\vec{\delta}_3\cdot\vec{k}}) & -M_c
\end{pmatrix}
\end{equation}
Diagolizing the above matrix, we achieve the eigenvalues of the $H_{MF}(\vec{k})$: $E_{\pm}(\vec{k}) = \pm \sqrt{\epsilon^2(\vec{k}) + M^2_c}$, where $\epsilon(\vec{k}) =  2t\sqrt{3+(\cos[(\vec{\delta}_1-\vec{\delta}_2)\cdot \vec{k}]+\cos[(\vec{\delta}_1-\vec{\delta}_3)\cdot \vec{k}]+\cos[(\vec{\delta}_2-\vec{\delta}_3)\cdot \vec{k}])}$ is the eigenvalues of the $H_0(\vec{k})$. The associated single-particle eigenstate of $H_{MF}(\vec{k})$ is denoted as $\beta^\dagger_{\pm}(\vec{k}) \ket{0}$. 

In the process of imaginary-time relaxation, the initial state, generated as the ground state of the MF Hamiltonian in \Eq{MFHam1}, evolves under the imaginary-time evolution of Hamiltonian in \Eq{NIHam1}. According to the scenario of ITME discussed in the main text, it is illuminating to evaluate the overlaps of the initial state with the eigenstates of the target Hamiltonian in \Eq{NIHam1} \sxz{S10}. In our study, we fix the number of electrons at half-filling, namely $N_e = N$ where $N$ is the number of unit cells. The ground state of \Eq{NIHam1} is written as the many-body wave function: $\prod_{\vec{k}} \alpha^\dagger_{-}(\vec{k}) \ket{0} $, where $\vec{k}$ belongs to the first Brillouin zone in which the total number of lattice momentum point is $N$. For the initial state under imaginary-time evolution, which is the ground state of MF Hamiltonian in \Eq{MFHam1}. The associated many-body wave function is written as: $\prod_{\vec{k}} \beta^\dagger_{-}(\vec{k}) \ket{0} $, where $\vec{k}$ belongs to the first Brillouin zone. Here, $\alpha_{-(+)}^\dagger(\vec{k})$ is the creation operator of an electron in the lower(higher)-energy single-particle eigenstate of $H_0(\vec{k})$, and $\beta_{-(+)}^\dagger(\vec{k})$ is the creation operator of an electron in the lower(higher)-energy single-particle eigenstate of $H_{MF}(\vec{k})$. The transformation between the eigenstates of the two Hamiltonian $\alpha_{-(+)}^\dagger(\vec{k})$ and $\beta_{-(+)}^\dagger(\vec{k})$ is given by:
\bea
\beta^\dagger_{-}(\vec{k}) &=& a_{-}(\vec{k}) \alpha^\dagger_{-}(\vec{k}) + b_{-}(\vec{k}) \alpha^\dagger_{+}(\vec{k}) \nonumber\\
\beta^\dagger_{+}(\vec{k}) &=& a_{+}(\vec{k}) \alpha^\dagger_{-}(\vec{k}) + b_{+}(\vec{k}) \alpha^\dagger_{+}(\vec{k})
\eea
Here, $(a_{-}(\vec{k}),b_{-}(\vec{k}))= \frac{1}{N_{-}}(1,-\frac{\sqrt{\epsilon^2(\vec{k})+M_c^2}-\epsilon(\vec{k})}{M_c})$ and $(a_{+}(\vec{k}),b_{+}(\vec{k}))= \frac{1}{N_{+}}(-\frac{\sqrt{\epsilon^2(\vec{k})+M_c^2}+\epsilon(\vec{k})}{M_c},1)$, where $N_{-} = \sqrt{1+\frac{(\sqrt{\epsilon^2(\vec{k})+M_c^2}-\epsilon(\vec{k}))^2}{M_c^2}}$ and $N_{+} = \sqrt{1+\frac{(\sqrt{\epsilon^2(\vec{k})+M_c^2}+\epsilon(\vec{k}))^2}{M_c^2}}$ are the normalized factors. It is straightfoward to show that $a_{-}(b_{-})$ decreases(increases) with $M_c$ monotonically, and in the limit $M_c = 0$, $a_{-}$ tends to one. Then we can evaluate the overlap between the MF initial states with finite $M_c$ and the different eigenstates of the evolution Hamiltonian $H_0$. The overlap of the MF state $\ket{\psi_{MF}}= \prod_{\vec{k}} \beta^\dagger_{-}(\vec{k}) \ket{0} $ with the ground state of $H_0$: $\ket{\psi_{0}}= \prod_{\vec{k}} \alpha^\dagger_{-}(\vec{k}) \ket{0} $, is $|c_0|^2 = \prod_{\vec{k}} |a_{-}(\vec{k})|^2 $, which decreases with increasing the value of $M_c$.
